Latent-Optimized Adversarial Neural Transfer for Sarcasm Detection

The existence of multiple datasets for sarcasm detection prompts us to apply transfer learning to exploit their commonality. The adversarial neural transfer (ANT) framework utilizes multiple loss terms that encourage the source-domain and the target-domain feature distributions to be similar while optimizing for domain-specific performance. However, these objectives may be in conflict, which can lead to optimization difficulties and sometimes diminished transfer. We propose a generalized latent optimization strategy that allows different losses to accommodate each other and improves training dynamics. The proposed method outperforms transfer learning and meta-learning baselines. In particular, we achieve 10.02% absolute performance gain over the previous state of the art on the iSarcasm dataset.

==> NAACL-HLT 2021 Latex Template/Chapters/Conclusion.tex <==
\section{Conclusion}

Transfer learning holds the promise for the effective utilization of multiple datasets for sarcasm detection. In this paper, we propose a latent  optimization (LO) strategy for adversarial transfer learning for sarcasm detection. By providing look-ahead in the gradient updates, the LO technique allows multiple losses to accommodate each other. This proves to be particularly effective in adversarial transfer learning where the domain-specific losses and the adversarial loss potentially conflict with one another. With the proposed LOANT method, we set a new state of the art for the iSarcasm dataset. We hope the joint utilization of multiple datasets will contribute to the creation of contextualized semantic understanding that is necessary for successful sarcasm detection. 
% Further, the success of LOANT underscores the importance of the interaction among multiple losses in the optimization of complex neural networks. 


% In this paper, we have studied transfer learning for improved sarcasm detection on human annotated datasets by making use of the automatically collected datasets. Our method is built on several recent advances in adversarial neural transfer, pretrained language models and meta learning. We propose a new effective adversarial neural transfer model based on latent-optimized BERT representations. We studied when to share the sarcasm classifier and BERT encoder under different transfer scenarios and examined the effectiveness and efficiency of adversarial learning and our proposed LO regularization. 



==> NAACL-HLT 2021 Latex Template/Chapters/Literature.tex <==
\section{Related Work}
\subsection{Sarcasm Detection}

% The task of automatic sarcasm or irony detection requires a model to have a strong feature extraction ability and a classifier to achieve good prediction performance on unseen data. Before the era of deep learning, the mainstream research in this field focus on finding better expressive features to improve classification performance through rule-based or context-aware methods. 



% With the advancement of computing power, pre-trained deep learning models are now widely adopted in NLP. models such as BERT are trained by integrating word embeddings and deep self-attention layers to automatically capture context, syntax and more complex linguistic patterns from a huge general corpora. These models possess big capacity in language understanding, demonstrating superior generalization performance than previous methods. However, fine-tuning such large pre-trained \textit{on-size-fit-all} models on small datasets incurs heavy overfitting problems and thus limits their power. 

Acquiring large and reliable datasets has been a persistent challenge for computational detection of sarcasm. Due to the cost of annotation, manually labeled datasets \cite{walker2012corpus,Riloff2013,wallace2014humans,abercrombie2016putting,oraby-etal-2016-creating,van2018semeval,oprea-magdy:2020:isarcasm} typically contain only a few thousand texts. Automatic crawling \cite{ptavcek2014sarcasm,bamman2015contextualized,joshi2015harnessing,khodak-etal-2018-large} using hashtags or markers yields substantially more texts, but the results are understandably more noisy. As a case study, after examining the dataset of \citeA{Riloff2013}, \citeA{oprea-magdy:2020:isarcasm} found that nearly half of tweets with sarcasm hashtags are not sarcastic. In this paper, we evaluate performance on the manually labeled datasets, which are relatively clean and can serve as good benchmarks, and transfer the knowledge learned from automatically collected datasets. 

% \hl{TODO: Cite \textbf{A LOT MORE} work on sarcasm detection. List \textbf{ALL} datasets and find out how many data points, the data source (twitter, reddit, etc), and the method of annotation. }

% The availability of the Twitter API makes it popular for tweets to be studied for sarcasm detection. The approaches to obtain labels for tweets are manual annotation and hashtag-based distant supervision. \cite{Riloff2013} introduced a dataset of 3,600 tweets manually annotated as sarcastic or not. \cite{ptavcek2014sarcasm} crawled a hash-tagged English dataset containing 100,000 tweets and a manually labeled Czech dataset containing 7,000 tweets. \cite{bamman2015contextualized} crawled a hash-tagged dataset evenly balanced at 19,534 English tweets, which contains authors' profile information and historical tweets for contextualized sarcasm detection. \cite{abercrombie2016putting} created a dataset of 2,240 two-line English tweets of which 448 were manually annotated as sarcastic conversations. \cite{tsur2010icwsm} collected a dataset of 6,6000 product reviews from Amazon.com of which 160 were manually annotated by third-party annotators for semi-supervised sarcasm detection. \cite{joshi2015harnessing} crawled a dataset of 9,378 English tweets using hashtags as labels. \cite{wallace2014humans} collected a manually labeled dataset of 3,020 comments from Reddit.com. \cite{khodak-etal-2018-large} crawled a dataset of 533 million Reddit comments of which 1.34 million having an $/s$ marker, which is the same as Twitter hashtags, to indicate sarcastic comments.

% \cite{walker2012corpus} crawled the Internet Argument Corpus containing 390,704 posts in 11,800 discussions from the online debate site 4forums.com, of which a subset of 2,254 were manually labeled as sarcastic posts. 

Traditional sarcasm detection includes methods based on rules \cite{tepperman2006yeah} and lexical \cite{kreuz-caucci-2007-lexical} and pragmatic patterns \cite{gonzalez2011identifying}. Context-aware methods \cite{rajadesingan2015sarcasm,bamman2015contextualized} make use of contexts, such as the author, the audience, and the environment, to enrich feature representations. 

Deep learning techniques for sarcasm detection employ convolutional networks \cite{ghosh2016fracking}, recurrent neural networks  \cite{zhang2016tweet,felbo-etal-2017-using,wu2018thu_ngn}, attention  \cite{tay-etal-2018-reasoning}, and pooling \cite{xiong2019sarcasm} operations. \citeA{amir2016modelling} incorporate historic information for each Twitter user. \citeA{cai-etal-2019-multi} consider the images that accompany tweets and \citeA{mishra-2017-gaze} utilize readers' gaze patterns. To the best of our knowledge, no prior work has explored transfer learning between different sarcasm datasets. 

% A recent study conducted a group test, of which half of the sarcastic tweets predefined by hashtags were relabeled as non-sarcastic by humans \cite{oprea-magdy:2020:isarcasm}. This indicates that even through we have a good sarcasm detection model, it may not work well in a new situation. In light of this, some researchers made efforts in creating human cross-validated datasets, including Riloff \cite{Riloff2013}, SemEval 2018 Task 3 \cite{van2018semeval} and iSarcasm \cite{oprea-magdy:2020:isarcasm}. Compared with hashtag labeled datasets, their sizes are ten times smaller. Different from single-task approaches designed for these small datasets, this paper aims to enhance sarcasm detection on these small datasets from the domain adaptation perspective. 

% Deep learning based methods have been employed in many NLP problems. In sarcasm detection, \cite{ghosh2016fracking} built a convolutional LSTM neural network for detecting sarcastic tweets. \cite{zhang2016tweet} combined Bi-GRU network extracted features and manually extracted context features for sarcasm detection. \cite{peled-reichart-2017-sarcasm} built a sequence-to-sequence model to translate a sarcastic sentence to non-sarcastic. \cite{felbo-etal-2017-using} built an attention-based Bi-directional LSTM for detecting sarcastic tweets using emojis and hashtags as supervision. \cite{wu2018thu_ngn} developed a densely connected LSTM neural network for predicting ironic labels, ironic types and ironic hashtags for a given tweet in a multi-task setting. \cite{tay-etal-2018-reasoning} combined the attention mechanism for extracting incongruous information and the LSTM neural network for compositional information extraction while \cite{xiong2019sarcasm} improved the concatenation of the two kinds of information by introducing a low-rank bilinear pooling to control information redundancy. \cite{cai-etal-2019-multi} extracted image features using ResNet and text features using Bi-LSTM for multi-modal sarcastic tweets detection. 

% However, little has been revealed by far on how to effectively utilize available scattered datasets via domain adaptation to boost performance on human supervised datasets without acquiring more costly labels. 

\subsection{Adversarial Transfer Learning}

% Domain Adaptation is the task in which a model aims to achieve success in a target domain with limited data and/or limited labels by exploiting knowledge learned from one or multiple source domains, given the fact that a systematic dataset shift exist between domains \cite{long2018conditional}. An earlier survey of transfer learning \cite{pan2009survey} categorized the domain adaptation problem as transductive transfer learning, where the assumption is that abundant labels are only available in source domain while the target is a different domain but the same task. In practice, the source and target domains are not mutually exclusive and they can have partial overlaps which requires efforts in finding suitable ways for domain adaptation. 

% Some surveys have organized existing domain adaptation research for different purposes. Surveys on domain adaptation for Neural Machine Translation (NMT) include \cite{chu2018survey} and \cite{li2012literature}. Surveys on domain adaptation for computer vision applications include both traditional and deep methods \cite{csurka2017domain} \cite{patel2015visual,wang2018deep}. Other related surveys cut the boundaries from the perspective of specific topics such as learning deep transferable features \cite{venkateswara2017deep}, multi-source domain adaptation \cite{sun2015survey}, zero-shot learning \cite{kodirov2015unsupervised} and unsupervised deep domain adaptation \cite{wilson2020survey}.

% Recent advances of deep domain adaptation methods leverage deep neural networks to learn transferable features that can generalize well to new domains. Adversarial adaptation methods have shown tremendous improvement towards this purpose by focusing on discovering domain-invariant features or mappings on shallow or high levels \cite{hoffman2018cycada}. The domain-invariant parameters are adversarially trained using a gradient reversal layer to be poor at domain classification; as a consequence, they produce representations that are domain agnostic. Most of existing deep adversarial domain adaptation methods borrow ideas from Generative Adversarial Networks (GANs) \cite{goodfellow2014generative}. Learning domain-invariant features via adversarial discriminators works similar as GANs in which the generator is any module that produces domain-invariant features. However, even with careful tuning, learning with adversarial networks may diverge or end up in a bad equilibrium with dropped modes without the balancing of delicate adversarial dynamics \cite{wu2019logan,pmlr-v80-balduzzi18a}. Besides, while domain adversarial networks yield reliable results for standard domain adaptation, there are occasions where they incur performance degeneration such as on the partial domain adaptation \cite{cao2019learning}. Thus, when and how to augment a model with what kind of adversarial module is tricky, often depending on dataset, domain discrepancy and learning task. If we are clear about this, it will save researchers and engineers from endless blind trials and go straight to pick a powerful adversarial learning technique to solve a given domain adaptation problem. 

As a transfer learning technique, multi-task learning (MTL) allows related tasks or similar domains to inform each other and has been a powerful technique for NLP \cite{Collobert2011,yang2017transfer,aharoni-etal-2019-massively,guo2019autosem,Raffel2020:T5}. However, MTL does not always lead to performance improvements \cite{alonso2017multitask,bingel-sogaard-2017-identifying,changpinyo2018multitask,clark2019bam}.

Theoretical analysis \cite{ben2010theory} indicates that a key factor for the success of transfer is to reduce the divergence between the feature spaces of the domains. \citeA{Ganin2015} propose to minimize domain differences via a GAN-like setup, where a domain discriminator network learns to distinguish between features from two domains and a feature extraction network learns to produce indistinguishable features, which are conducive to transfer learning.

Similar adversarial setups \cite{liu-etal-2017-adversarial,kim2017adversarial} have been adopted for many NLP tasks, such as sentiment analysis \cite{chen2018adversarial,liu2018learning}, satirical news detection \cite{mchardy-etal-2019-adversarial}, detection of duplicate questions \cite{kamath2019reversing}, named entity recognition \cite{zhou2019dual_c}, and QA \cite{YuJianfei2018}. 

However, as shown in our experiments, adding the domain discriminator to MTL does not always result in improved performance. We attribute this to the implicit competition between the negative domain discrimination loss and the domain-specific losses, which causes difficulties in optimization. In this paper, we improve the training dynamics of adversarial transfer learning using latent optimization on BERT features.


% Adversarial domain adaptation methods in NLP are mainly application-driven. For example, cross-lingual sentiment classification utilizes adversarial network to map shared sentiment features across languages to the same feature space \cite{chen2018adversarial}. This can be further applied to multi-source sentiment classification in which more existing resources are used to improve sentiment analysis in low-resource languages \cite{liu2018learning}. In other scenarios, adversarial networks can also be used to eliminate the influence of confounding variables (variables that have correlation with observed variables and this can mislead hypothesis model to make predictions) in satire detection \cite{mchardy-etal-2019-adversarial} and in duplicate question detection \cite{kamath2019reversing}. Neural network models designed under multi-task learning framework focus on learning the shared layers to extract the common and task-invariant features. The shared features are prone to be contaminated by label noise and exclusive features from other related tasks. Adversarial multi-task learning framework introduces an adversarial network by forcing the feature extraction module to learn domain-invariant feature space \cite{liu-etal-2017-adversarial}. 


\subsection{Meta-Learning and Latent Optimization}
The idea of coordinating gradient updates of different and competing losses using gradient descent with look-ahead has been explored in Latent-optimized Generative Adversarial Network (LOGAN) \cite{pmlr-v97-wu19d,wu2019logan}, Symplectic Gradient Adjustment \cite{Balduzzi2018:n-Player,gemp2019global}, Unrolled GAN \cite{metz2016unrolled}, Model-Agnostic Meta Learning \cite{pmlr-v70-finn17a} and extragradient \cite{azizian2020:extragradient}. The difference between LOGAN and other techniques is that the LOGAN computes the derivative of the randomly sampled latent input, whereas other methods compute the second-order derivative in the model parameter space. 

In this paper, we generalize latent optimization from GANs to multi-task learning, where the adversarial loss is complemented by domain-specific task losses. In addition, we apply latent optimization on the output of the BERT module, which differs from the optimization of the random latent variable in LOGAN. As large pretrained masked language models (PMLMs) gain prominence in NLP, latent optimization avoids gradient computation on the parameters of enormous PMLMs, providing reduction in running time and memory usage. 


% has provided a general framework for model transfer across a number of tasks . It is worth noting that meta learning in latent optimization is to optimize latent variables instead of the whole model parameters . The advantage is a big reduction on computation complexity with a little sacrifice of model expressiveness.


% Latent optimization has been shown to improve the GAN dynamics and the final performance in image generation. However, we found that potential of latent optimization remains untapped in adversarial domain adaptation and its applications in NLP. In this paper, we ground the general latent optimization in the adversarial domain adaptation framework and study its effectiveness and efficiency under both supervised and unsupervised learning settings.


% Model adaptation methods share a similar idea as domain adaptation methods in which the intuition is to consider possible discrepancies when establishing a hypothesis model so that the final model is able to tolerate certain practical bias. The difference is that domain adaptation methods are restricted by working on similar tasks while model adaptation methods treat all tasks as learning examples and the final model is (ideally) universal. Research on meta learning and heterogeneous horizontal federated learning fall in this category.

% The notion of learning to learn, or meta-learning \cite{hochreiter2001learning} inspired a lot of research on automatic adaptation of models learned with gradient descent methods \cite{andrychowicz2016learning,pmlr-v70-finn17a}. Meta-learning in neural networks can be seen as aiming to provide the gradient descent optimization with next step of integrating joint feature, model, and algorithm learning. This paradigm is related to the field of transfer learning except that meta learning do not have a prerequisite of similar tasks. 



% In particular, This learning-to-learn strategy has the potential to alleviate many criticisms \cite{marcus2018deep} of contemporary deep learning by improving knowledge transfer and unsupervised learning in both multi-task and single-task scenarios.


% On the application side, meta learning has been widely evaluated in architecture search \cite{zoph2018learning}, activation functions search \cite{ramachandran2017searching}, latent optimization \cite{rusu2018meta}, etc, mainly in the field of computer vision. It is worth noting that meta learning in latent optimization is to optimize latent variables instead of the whole model parameters \cite{pmlr-v97-wu19d,wu2019logan}. The advantage is a big reduction on computation complexity with a little sacrifice of model expressiveness. Compared with searching for whole model parameters, latent optimization only considers optimization cost on a given latent variable, leaving the rest parameters optimized as usual. It was recently proved in GANs to refine latent source sampled from random space for compressed sensing \cite{pmlr-v97-wu19d} and image generation \cite{wu2019logan}. 
